Simultaneous Localization and Mapping: Through the Lens of Nonlinear Optimization

Simultaneous Localization and Mapping (SLAM) algorithms perform visual-inertial estimation via filtering or batch optimization methods. Empirical evidence suggests that filtering algorithms are computationally faster, while optimization methods are more accurate. This work presents an optimization-based framework that unifies these approaches, and allows users to flexibly implement different design choices, e.g., the number and types of variables maintained in the algorithm at each time. We prove that filtering methods correspond to specific design choices in our generalized framework. We then reformulate the Multi-State Constrained Kalman Filter (MSCKF), implement the reformulation on challenging image sequence datasets in simulation, and contrast its performance with that of sliding window based filters. Using these results, we explain the relative performance characteristics of these two classes of algorithms in the context of our algorithm. Finally, we illustrate that under different design choices, the empirical performance of our algorithm interpolates between those of state-of-the-art approaches.

==> Alg___sliding_window.tex <==

% \newpage

% \frank{To edit, e.g., dimensions}



\begin{algorithm} \label{Alg: Generalized Sliding Window Filter}
    {
    % \normalsize
    \small
    % \footnotesize
    \SetAlgoLined
    \KwData{Prior on $x_{\IMU,0} \in \X_p$: $\mathcal N(\mu_0, \Sigma_0)$, noise covariances $\Sigma_w
    % \in \R^{\dx \times \dx}
    $, $\Sigma_v
    % \in \R^{d_ \times d_z}
    $, dynamics $g_\IMU
    % : \X_\IMU \times \X_\IMU
    $, measurement map $h
    % : \X_p \times \R^{\df} \ra \R^{d_z}
    $, time horizon $T$, pose transformation $\psi$ (IMU $\ra$ global).}
    
    \KwResult{Estimates $\hat x_t 
    % \in \X_\IMU \times (\X_p)^n \times (\R^{\df})^{\nf}
    , \hspace{0.5mm} \forall \hspace{0.5mm} t \in \{1, \cdots, T\}$
    % , where $n:=$ number of poses in $\hat{x}_t$ at time $t$
    .} 
    
    % \frank{To edit below:}
    % $\nf \gets 0$
    % \vspace{2mm} 
    % \textcolor{red}{\textbf{To edit, below:}}
    
    $\cost_t \leftarrow \Vert x_0 \boxminus \mu_0 \Vert_{\Sigma_0}^2 \in \R$. (Initialize objective function).
    
    $x_0^\star \leftarrow \mu_0 \in \X_p$. (Initialize linearization point).
    
    $S_z, S_x, S_{z,1}, S_{z,2} \gets \phi$ 
    
    $(\nx, \nf) \gets (0, 0)$ 
    
     \For{$t = 0, \cdots, T$}{
     
        % \frank{(1)}

        $x_{\nx +1} \in \X_p \gets$ New pose recorded in new image
        
        % , new IMU measurement not received
        
            $\cost_t \leftarrow \cost_t + \epsilon^{-1} \Vert x_{\nx +1} \boxminus \psi(\tilde{x}_t, x_{\nx +1}^\IMU) \Vert_2^2 \in \R$.
            
            $\mu_t
            % \in \X_\IMU \times (\X_p)^n \times (\R^{\df})^{\nf}
            , \Sigma_t
            % \in \R^{(d_\IMU + n \dx + \nf \df) \times (d_\IMU + n \dx + \nf \df)}
            , \cost_t \gets $ Gauss-Newton step(s) on $\cost_t$, about $\big(\mu_t, \psi(\mu_t, x_{\nx +1}^\IMU)\big)$ (Alg. \ref{Alg: gauss-newton}), with $\epsilon \ra 0$
            
            % \frank{(2)}
            
            % $z_{t,\nf+1:\nf+\nf'} \gets (z_{t,\nf+1}, \cdots, z_{t,\nf+\nf'}) \in \R^{\nf' d_z} \gets$ New measurements of new features

            % $\text{cost}_t \gets \text{cost}_t + \sum_{k= \nf+1}^{\nf+\nf'} \|z_{t,k} - h(x_t, f_k)\|_{\Sigma_{v}^{-1}}^2 \in \R.$
            
            % \frank{(2,3)}
            
            $(z_{t,1}, \cdots, z_{t,\nf+\nf'}) 
            % \in \R^{(\nf+\nf')d_z}
            \gets$ Measurements of existing features.            
            
            $\text{cost}_t \gets \text{cost}_t + \sum_{k=1}^{\nf+\nf'} \|z_{t,k} - h(x_t, f_k)\|_{\Sigma_{v}^{-1}}^2 \in \R.$
  
          $\overline\mu_t 
        %   \in \X_\IMU \times (\X_p)^n \times (\R^{\df})^{\nf}
          , \overline\Sigma_t 
        %   \in \R^{(d_\IMU + n \dx + \nf \df) \times (d_\IMU + n \dx + \nf \df)}
          , \text{cost}_t \gets$ Gauss-Newton step(s) on $\cost_t$, about $\mu_t$, 1 iteration
          (Alg. \ref{Alg: gauss-newton}
        %   , Theorem \ref{Thm: EKF Update}
        ).
            
            % \frank{INCOMPLETE: Pose Augmentation algorithm subblock}
            
            
            
        %     $S_z \gets S_z \cup \big\{ (x_{\nx +1}, f_{j})| \text{ Feature } j \text{ observed at $n+1$} \big\}$ 
            
        %     $n \gets n+1$
        
        % \If{$n \geq N_{\max}-1$}{
        
        %     $S_x \gets \{x_i | i \text{ mod } 3 = 2, \text{ and } 1 \leq i \leq n. \}$
            
        %     $S_{z,1} \gets \big\{ (x_i, f_{j}) \in S_z \big| x_i \in S_x, \text{feature $j$ observed at each pose in } S_x \big\}$
        % }
        
        % $S_{z,2} \gets \big\{ (x_i, f_{j}) \in S_z | x_i \in x_{1:n}, \text{feature } j \text{ observed at } x_i \text{ but not at } x_n \big\}$.
        
        % \frank{(4)}
        
        $S_x \gets \{x_i | x_i \text{ is a pose to marginalize} \}$
        
        $\overline\mu_t 
        % \in \X_\IMU \times (\X_p)^n \times (\R^{\df})^{\nf}
        , \overline\Sigma_t 
        % \in \R^{(d_\IMU + n \dx + \nf \df) \times (d_\IMU + n \dx + \nf \df)}
        , \cost_t \gets$ Marginalization step on $\cost_t$, about $\mu_t$ (Alg. \ref{Alg: marginalization}).
        % , with $x_M := $ Concatenation of poses in $S_x$, $x_K := $ Concatenation of other components of $\tilde{x}_t$
        
        % \frank{(5)}
        
        $S_z \gets \big\{ (x_i, f_{j}) \big| \text{Feature measurements to marginalize} \big\}$
        
        $S_f \gets \big\{ f_{j} \big| \exists \hspace{0.5mm} x_i \in x_{1:n} \text{ s.t. } (x_i, f_{j}) \in S_z \big\}$
        
            $\cost_t \leftarrow \cost_t + \sum_{(x_i, f_j) \in S_z} \Vert z_{i,j} \boxminus h(x_i, f_j) \Vert_{\Sigma_v^{-1}} \in \R$
            
            $\overline{\mu_t} 
            % \in \X_\IMU \times (\X_p)^n \times (\R^{\df})^{\nf}
            $, $\overline{\Sigma_t}
            % \in \R^{(d_\IMU + n \dx) \times (d_\IMU + n \dx)}
            $, $\cost_t \gets$ Gauss-Newton step(s) on $\cost_t$ (Alg. \ref{Alg: gauss-newton})
            
            % $\overline{\mu_t}, \overline{\Sigma_t} \gets $ Alg. \ref{Alg: MSCKF, Feature Update Sub-block} ($\tilde{x}_t$, $\mu_t$, $\Sigma_t$, $x_{\nx +1}$, $S_z$, $S_f$, $h(\cdot)$)
            
            % \frank{INCOMPLETE: Feature Update algorithm subblock}
            
            $\hat x_t \gets \overline{\mu_t} \in \X_\IMU \times (\X_p)^n \times (\R^{\df})^{\nf}$.
        
        % $S_z \gets S_z \backslash (S_{z,1} \cup \{(x_i, f_j) | x_i \in S_x \})$
        
        Reindex poses and features, in ascending order
        % of index, i.e., $\{x_1, \cdots, x_{\nx -|S_x|}\}$ and $\{f_1, \cdots, f_{\nf -|S_f|}\}$
        .
        
        
        $(\nf,n) \gets (\nf-|S_f|, \nx -|S_x|)$
        
        % Reindex features, in ascending order of index, as .
        
        % \vspace{2mm}
        
        % \frank{(6)}
        
        \If{$t < T$}{
        
            $\cost_t \gets \cost_t + \Vert x_{t+1, \IMU} \boxminus g_\IMU(x_{t,\IMU}) \Vert_{\Sigma_w^{-1}}^2 \in \R$.
        
            $\mu_{t+1} 
            % \in \X_\IMU \times (\X_p)^n \times (\R^{\df})^{\nf}
            , \Sigma_{t+1} 
            % \in \R^{(d_\IMU + n \dx + \nf \df) \times (d_\IMU + n \dx + \nf \df)}
            , \cost_t \gets$ Marginalization step on $\cost_t$, about $\big(\mu_{t,\IMU}, g_\IMU(\mu_{t,\IMU}) \big)$ (Alg. \ref{Alg: marginalization})
            
            % \frank{INCOMPLETE: State Propagation algorithm subblock}
        
        }
     }
    
    \Return{$\hat x_0, \cdots \hat x_T \in \X_\IMU \times (\X_p)^n \times (\R^{\df})^{\nf}$}
     
     \caption{Generalized Sliding Window Filter, as an iterative optimization problem 
    %  \frank{Rough Draft}
     .}
     }
\end{algorithm}


% \begin{algorithm} 
% % \label{Alg: Generalized Sliding Window Filter}
%     {\scriptsize
%     \SetAlgoLined
%     \KwData{Prior distribution on $x_0 \in \R^{\dx}$: $\mathcal N(\mu_0, \Sigma_0)$, dynamics and measurement covariances $\Sigma_w \in \R^{\dx \times \dx}, \Sigma_v \in \R^{d_ \times d_z}$, dynamics map $g: \R^{\dx} \times \R^{\dx}$, measurement map $h: \R^{\dx} \times \R^{\df} \ra \R^{d_z}$, time horizon $T$.}
%     \KwResult{Estimates $\hat x_t$ for all desired timesteps $t \leq T$.}
    
%     $\nf \gets 0$
    
%     % \vspace{2mm} 
%     % \textcolor{red}{\textbf{To edit, below:}}
    
%      \For{$t = 0, \cdots, T$}{
%         $\nx' \gets \min\{t+1, n\}$.
        
%         \If{\textbf{\emph{detect new feature measurements}} $z_t := (z_{t,\nf+1}, \cdots, z_{t,\nf+\nf'}) \in \R^{\nf' d_z}$}{
     
%         $(\mu_{t,x,t-n+1}, \cdots, \mu_{t,x,t}, \mu_{t, f, 1:\nf}) \gets \mu_t \in \R^{\nx' \dx + \nf \df}$, with $\mu_{t,x,t-n+1}, \cdots, \mu_{t,x,t} \in \R^{\dx}$, $\mu_{t, f, 1:\nf} \in \R^{\nf \df}$.
     
%         $\ell: \R^{\dx} \times \R^{d_z} \ra \R^{\df} \gets$ Inverse measurement map, satisfying $z_{t,k} = h \big( x_t, \ell(x_t, z_{t,k}) \big)$ for each $x_t \in \R^{\dx}$, $z_{t,k} \in \R^{d_z}$, $\forall \hspace{0.5mm} k = 1, \cdots, \nf$.
        
%         $\tilde{\ell}(\mu_{t,x,t}, z_{t,\nf+1}, \cdots, z_{t,\nf+\nf'}) \gets \big( \ell(\mu_{t,x,t}, z_{t,\nf+1}), \cdots, \ell(\mu_{t,x,t}, z_{t,\nf+\nf'}) \big) \in \R^{(\nf' \df) \times (\dx + \nf' d_z)}$
        
%         $\mu_t \gets \big(\mu_t, \tilde{\ell}(\mu_{t,x,t}, z_{t,\nf+1}, \cdots, z_{t,\nf+\nf'}) \big) \in \R^{\nx' \dx + (\nf+\nf')\df}$
        
%         $\begin{bmatrix}
%         \Sigma_{t,xx} & \Sigma_{t,xf} \\
%         \Sigma_{t,fx} & \Sigma_{t,ff} 
%         \end{bmatrix} \gets \Sigma_t \in \R^{(\nx' \dx + \nf \df) \times (\nx' \dx + \nf \df)}$, with $\Sigma_{t,xx} \in \R^{\nx' \dx \times \nx' \dx}$, $\Sigma_{t,xf} = \Sigma_{t,fx}^\top \in \R^{\nx' \dx \times \nf \df}$, $\Sigma_{t,ff} \in \R^{\nf \df \times \nf \df}$.
        
%         $L_x \gets \frac{\partial \tilde{\ell}}{\partial x} \big|_{(\mu_t, z_t')} \in \R^{\nf' \df \times \dx}$
        
%         $L_z \gets \frac{\partial \tilde{\ell}}{\partial z} \big|_{(\mu_t, z_t')} \in \R^{\nf' \df \times d_z}$
        
%         $\tilde{\Sigma}_v \gets \text{diag}\{\Sigma_v, \cdots, \Sigma_v\} \in \R^{\nf' d_z \times \nf' d_z}$
        
%         $\Sigma_t \gets \begin{bmatrix}
%         \Sigma_{t,xx} & \Sigma_{t,xf} & \Sigma_{t,xx} L_x^\top \\
%         \Sigma_{t,fx} & \Sigma_{t,ff} & \Sigma_{t,fx} L_x^\top \\
%         L_x \Sigma_{t,xx} & L_x \Sigma_{t,xf} & L_x \Sigma_{t,xx} L_x^\top + L_z \tilde{\Sigma}_v L_z^\top
%         \end{bmatrix} \in \R^{(\dx + (\nf+\nf')\df) \times (\dx + (\nf+\nf')\df)} $
        
%         $\nf \gets \nf + \nf'$
%         }
        
%         % \vspace{2mm}
        
%         $z_{t,1:\nf} \gets (z_{t,1}, \cdots, z_{t,\nf}) \in \R^{ \nf d_z}$ $\hspace{1cm}$ (New measurements)
        
%         $z_{t-\nx'+1:t} \gets (z_{t-\nx'+1}, \cdots, z_t) \in \R^{\nx' d_z}$
        
%         ${\nf}_m \in \{0,1, \cdots, \nf\} \gets$ Number of features not seen by current pose.
        
%         \If{${\nf}_m \geq 1$}{
            
%             Reindex features, with those not observed at current pose as $\{\nf -{\nf}_m+1, \cdots, \nf\}$.
            
%             $z_{t,\nf -{\nf}_m+1:\nf} \gets (z_{t,\nf -{\nf}_m+1}, \cdots, z_{t,\nf}) \in \R^{{\nf}_m d_z}$.
            
%             $\overline{x_t} \gets (x_{t-\nx'+1}, \cdots, x_t, f_{t,1}, \cdots, f_{t,\nf -{\nf}_m}) := (x_{t-\nx'+1:t}, f_{t,1:\nf -{\nf}_m}) \in \R^{\nx' \dx + (\nf-{\nf}_m) \df}$.
            
%             $f_{t,\nf -{\nf}_m+1:\nf} \gets (f_{t,{\nf}_m+1}, \cdots, f_{t,\nf}) \in \R^{\df {\nf}_m}$
            
%             % \If{${\nf}_m \leq \nf -1$}{
                
%             % }
%             $\Tilde{h}(\overline{x_t}) \gets \big( h(x_{t-\nx'+1}, f_{t,1}), \cdots, h(x_t, f_{t,1}), \cdots, h(x_{t-\nx'+1}, f_{t,\nf}), \cdots, h(x_t, f_{t,\nf}) \big) \in \R^{\nx' \nf d_z}$.
            
%             $\tilde{H}_{t,x} \gets \frac{\partial}{\partial \overline{x_t}} \Tilde{h}(\overline{x_t}, f_{t,1:\nf -{\nf}_m}) \Big|_{\mu_t} \in \R^{\nx' \nf d_z \times (\nx' \dx + (\nf-{\nf}_m)\df)}.$ 
%             % \in \R^{\nx qd_z \times n \dx}.
            
%             $\tilde{H}_{t,f} \gets \frac{\partial}{\partial f_{t,\nf -{\nf}_m+1:\nf}} \tilde{h}(\overline{x_t}, f_{t,\nf -{\nf}_m+1:\nf}) \Big|_{\mu_t} \in \R^{\nx' \nf d_z \times {\nf}_m \df}.$
%             % \in \R^{\nx qd_z \times \nf \df}.
            
%             $\mu_t \gets \begin{bmatrix}
%                 I_{\nx' \dx + (\nf-{\nf}_m) \df} & O
%             \end{bmatrix} \mu_t$.
            
%             $\Sigma_t \gets \begin{bmatrix}
%                 I_{\nx' \dx + (\nf-{\nf}_m) \df} & O
%             \end{bmatrix} \Sigma_t \begin{bmatrix}
%                 I_{\nx' \dx + (\nf-{\nf}_m) \df} \\ O
%             \end{bmatrix} $.
            
%             $\{a_1, \cdots, a_{\nx' \nf d_z - {\nf}_m \df}\} \subset \R^{\nx' qd_z} \gets \text{ Orthonormal basis for } N(\tilde{H}_{t,f}^\top).$
            
%             $A \gets \begin{bmatrix}
%             a_1 & \cdots & a_{\nx' \nf d_z - {\nf}_m \df}
%             \end{bmatrix} \in \R^{\nx'  \nf d_z \times (\nx' \nf d_z - {\nf}_m \df)}$
            
%             % \label{Eqn: Generalized Sliding Window Filter, QR decomposition of A transpose Hx}
%             $QT \gets$ QR Decomposition of $A^\top \tilde{H}_{t,x}$, with $Q \in \R^{(\nx' \nf d_z - {\nf}_m \df) \times (\nx' \nf d_z - {\nf}_m \df)}$, $T \in \R^{(\nx' \nf d_z - {\nf}_m \df) \times (\nx' \dx + (\nf-{\nf}_m)\df)}$.
            
%             % Jacobian of $h$ w.r.t. $f_{t,1:\nf}$ evaluated at $\mu_t$.
            
%             % \label{Eqn: Generalized Sliding Window Filter, Covariance Update}
%             $\overline{\Sigma}_t^{-1} \gets \Sigma_t^{-1} + T^\top (Q^\top A^\top RAQ)^{-1} T \in \R^{(\nx' \dx + (\nf-{\nf}_m)\df) \times (\nx' \dx + (\nf-{\nf}_m)\df)}$.
            
%             % \label{Eqn: Generalized Sliding Window Filter, Mean Update}
%             $\overline{\mu_t} \gets \mu_t + \big( \Sigma_t^{-1} + T^\top (Q^\top A^\top RAQ)^{-1} T \big)^{-1} T^\top (Q^\top A^\top R AQ)^{-1} \big(z_{t-\nx'+1:t} - \Tilde{h}(\overline{x_t}) \big) \in \R^{\nx' \dx + (\nf-{\nf}_m) \df}$.
            
%             $\hat x_t \gets \overline{\mu_t} \in \R^{\nx' \dx + (\nf-{\nf}_m) \df}$.
            
%             $\nf \gets \nf -{\nf}_m$
        
%         }
        
%         % \vspace{2mm}
%         \If{$t < T$}{
%             $\tilde{g}(\overline{x_t}) \gets \big(g(x_{t-n+1}), \cdots, g(x_t), f_{t,1}, \cdots, f_{t,\nf} \big) \in \R^{\nx' \dx + \nf \df}$
            
%             $\tilde{G_t} \gets \frac{\partial \tilde{g}}{\partial \overline{x_t}} \Big|_{\overline{\mu_t}} \in \R^{(\nx' \dx + \nf \df) \times (\nx' \dx + \nf \df)}$
            
%             % $G_t \in \R^{(\nx' \dx + \nf \df) \times (\nx' \dx + \nf \df)} \gets $ Jacobian of $g: \R^{\nx' \dx + \nf \df} \ra \R^{\nx' \dx + \nf \df}$, evaluated at $\overline{\mu_t} \in \R^{\nx' \dx + \nf \df}$.
        
%             $\mu_{t+1} \gets \tilde{g}(\overline{\mu_t}) \in \R^{\nx' \dx + \nf \df}$.
            
%             $\Sigma_{t+1} \gets \tilde{G}_t \overline{\Sigma}_t \tilde{G}_t^T + \Sigma_w \in \R^{(\nx' \dx + \nf \df) \times (\nx' \dx + \nf \df)}$.
%         }
        
%      }
    
%     \Return{$\hat x_0, \cdots \hat x_T \in \R^{\nx' \dx + (\nf-{\nf}_m) \df}$}
     
%      \caption{Generalized Sliding Window Filter, as an iterative optimization problem.}
%      }
% \end{algorithm}
